Resonance based schemes for SPDEs

Resonance based numerical schemes are those in which cancellations in the oscillatory components of the equation are taken advantage of in order to reduce the regularity required of the initial data to achieve a particular order of error and convergence. We investigate the potential for the derivation of resonance based schemes in the context of nonlinear stochastic PDEs. By comparing the regularity conditions required for error analysis to traditional exponential schemes we demonstrate that at orders less than $ \mathcal{O}(t^2) $, the techniques are successful and provide a significant gain on the regularity of the initial data, while at orders greater than $ \mathcal{O}(t^2) $, that the resonance based techniques does not achieve any gain. This is due to limitations in the explicit path-wise analysis of stochastic integrals. As examples of applications of the method, we present schemes for the Schr\"odinger equation and Manakov system accompanied by local error and stability analysis as well as proof of global convergence in both the strong and path-wise sense.

==> glossary.tex <==
\newglossaryentry{set_of_trees}{
	name={\ensuremath{\hat{\mathscr{T}}}},
	description={Set of decorated trees.}
}

\newglossaryentry{tree_to_integral}{
	name={\ensuremath{\Pi}},
	description={A character mapping decorated trees, specifically elements of \gls{span}, to iterated integrals in \gls{iterated_integrals}}}

\newglossaryentry{forest}{
	name={\ensuremath{\hat{H},\hat{H}_0}},
	description={Unordered forests composed of trees in \gls{set_of_trees} or \gls{set_of_decorated-trees_no-time} respectively}
}

\newglossaryentry{span}{
	name={\ensuremath{\hat{\mathscr{H}}, \hat{\mathscr{H}}_0  }},
	description={The Linear span of \gls{forest} }
}

\newglossaryentry{graft}{%
	name={ \ensuremath{\mathscr{T_{(\mathfrak{t}, \mathfrak{p})}(\lambda_k^l\cdot)}}}, 
	description={An operation interpreted as merging all of the roots of trees composing a forest into one node decorated by $ (l,k) \in \NN \times \ZZ^d $}
}

\newglossaryentry{K_operator}{%
	name={ \ensuremath{\mathscr{K}} }, 
	description={Computes an approximation of the integrals introduced via iterations of Duhamel's formula}
}

\newglossaryentry{iterated_integrals}{
	name={\ensuremath{\mathscr{C}} },
	description={Space of oscillatory integrals}
}

\newglossaryentry{differential_parameters}{
	name={\ensuremath{\mathfrak{L}}},
	description={A finite set which parametrises a set of differential operators with constant coefficients whose symbols are given by the polynomials \ensuremath{(P_\tf)_{\tf\in\Lf}}}
}

\newglossaryentry{tree_element}{
	name={ \ensuremath{T^{\mathfrak{n}, \mathfrak{f}}_\mathfrak{e}} },
	description={An element of \gls{set_of_trees} with edge decorations \gls{edge_decoration}, node decorations for time monomials \gls{time_decoration} and node decorations for the frquencies \gls{frequencies}}
}


\newglossaryentry{tree_element_no-time}{name={\ensuremath{T_\mathfrak{e}^\mathfrak{f}}},description={Decorated trees with node decorations $ \nf $ all equal to zero}}


\newglossaryentry{edge_decoration}{
	name={\ensuremath{\mathfrak{e}}},
	description={Maps edges $ E_T $ to \gls{differential_parameters}$ \times \{0,1\} $}
}


\newglossaryentry{time_decoration}{
	name={\ensuremath{\mathfrak{n}}},
	description={encodes a monomial}
}


\newglossaryentry{frequencies}{
	name={\ensuremath{\mathfrak{f}}},
	description={frequencies}
}


\newglossaryentry{tree}{
	name={\ensuremath{T}},
	description={A nonplanar rooted tree with root $ \varrho_T $, node set $ N_T $ with leaves $ L_T $ and edge set $ E_T $}
}
\newglossaryentry{node_decorations}{name={\ensuremath{N_T}},description={Node decorations encoding monomials of the time variable}}

\newglossaryentry{decorated_trees_generated_by_R}{name={\ensuremath{\hat{\mathscr{T}}_0(R)}}, description={Set of decorated trees generated by $ R $.}}

\newglossaryentry{order_projection}{name={\ensuremath{\mathscr{D}^r}},description={Replaces the root decoration of a tree with $ r $ and projects along the identity. Extended multiplicitively to forests it projects according to the order of the scheme $ r $, disregarding trees of higher degree}}


\newglossaryentry{root_node}{name={\ensuremath{\varrho_T}},description={Root node of a tree}}


\newglossaryentry{edge_set}{name={\ensuremath{E_T}},description={Set of edges of trees}}


\newglossaryentry{leaf_set}{name={\ensuremath{L_T}},description={Leaves of the tree $ T $}}


\newglossaryentry{set_of_decorated-trees_no-time}{name={\ensuremath{\hat{\mathscr{T}}_0}},description={Set of decorated trees with $ \nf=0 $}}

%\newglossaryentry{subtree}{name={\ensuremath{\overline{T}_{\overline{\mathfrak{e}}}^{\overline{\mathfrak{f}}}}},description={A decorated subtree of $ T^{\tf}_\ef $}}


\newglossaryentry{decorated_edge}{name={\ensuremath{\mathscr{I}_o}},description={Denotes an edge decorated by $ o=(\tf,\ff) $}}

\newglossaryentry{approximation_Pi}{name={\ensuremath{\Pi^n}},description={Low regularity approximation to $ \Pi $}}

\newglossaryentry{approximated_trees}{name={\ensuremath{\mathscr{T}}},description={The set of approximated decorated trees}}
	
\newglossaryentry{decorated_tree}{name={\ensuremath{T_{\mathfrak{e}, r}^{\mathfrak{n}, \mathfrak{f}}}},description={An approximation of order $r$ to the decorated tree $T_{\ef}^{\nf,\ff}$}}

\newglossaryentry{dominant_polynomial}{name={\ensuremath{\mathscr{P}_{\text{dom}}(P)}},description={The highest order term of the resonance structure, the term contains the dominant frequency.}}
